Linear Transformer Topological Masking with Graph Random Features

When training transformers on graph-structured data, incorporating information about the underlying topology is crucial for good performance. Topological masking, a type of relative position encoding, achieves this by upweighting or downweighting attention depending on the relationship between the query and keys in a graph. In this paper, we propose to parameterise topological masks as a learnable function of a weighted adjacency matrix -- a novel, flexible approach which incorporates a strong structural inductive bias. By approximating this mask with graph random features (for which we prove the first known concentration bounds), we show how this can be made fully compatible with linear attention, preserving $\mathcal{O}(N)$ time and space complexity with respect to the number of input tokens. The fastest previous alternative was $\mathcal{O}(N \log N)$ and only suitable for specific graphs. Our efficient masking algorithms provide strong performance gains for tasks on image and point cloud data, including with $>30$k nodes.

==> discussion.tex <==
\section{Discussion}

\textcolor{blue}{[Bits and bobs we could insert somewhere. Some are already integrated.]}

We conclude with the following series of remarks. 

\pg{GRFs give sparse masks}
We have seen that GRFs are sparse even though their dot product accurately approximates a Taylor mask $\mathbf{M}_\alpha(\mathcal{G})_{ij}$ with high probability. 
\vspace{0.5mm}It follows that the implicit topological mask \smash{${\widehat{\mathbf{M}}_\alpha} \coloneqq  [\widehat{\phi}_\mathcal{G}(v_i)^\top \widehat{\phi}_\mathcal{G}(v_j) ]_{i,j=1}^N$}, which is never materialised in memory, is also sparse. 
Whilst attentive sparsity is often invoked to improve efficiency \citep{child2019generating, kitaev2020reformer}, it rarely actually \emph{improves} predictive performance.
This is testament to the strong inductive bias GRFs provide: the benefits of topological masking outweigh the fact that each token can can attend to fewer tokens compared to the unmasked case.
The sparsity of \smash{$\widehat{\mathbf{M}}_\alpha$} also offers a new way to learn to speed up computation of \emph{full-rank} attention, which we aim to explore in future work.

\textbf{Analogy to RoPE} \citep{su2024roformer}\textbf{.}
Rotary Positional Embeddings (RoPE) is a positional embedding technique popular in the natural language processing community, used in large language models like LLama, LLama2, PaLM and CodeGen. 
It works by separately rotating the query and key vectors by an angle that depends on their respective tokens' absolute positions, such that the modification to the dot product depends on the positional difference.
This combines the strengths of absolute and relative position encoding: on the one hand, encodings are efficiently computed for individual queries and keys and are not changed when new tokens are generated, making RoPE compatible with KV-caching; on the other hand, the attention modulation is a function of distance between tokens so sensibly captures their spatial relationship. 
Our algorithm shares these properties. 
GRFs are computed independently for every token, but when combined reflect a mathematically principled notion of their relative positions by estimating a graph node kernel. 

\pg{GRFs close the performance gap between linear and softmax attention} \textcolor{blue}{Something about capturing spikes and abilility to sharply upweight and downweight attention evaluations. \citep{clark2019does}, capturing big spikes in attention. I'm struggling to find good references for this but think it's well known that this is why softmax is good.}


==> old.tex <==
\begin{figure}[h!]
\centering
\begin{minipage}{0.6\textwidth}
    \centering
    \begin{tabular}{cccc}
    \makecell{\emph{\small{Groundtruth}} \\ \emph{\small{video frame}}} & 
    \adjustbox{valign=m}{\includegraphics[width=1.5cm]{iclr2024/renderings/groundtruth/videoframe_0.png}} & 
    \adjustbox{valign=m}{\includegraphics[width=1.5cm]{iclr2024/renderings/groundtruth/videoframe_106.png}} & 
    \adjustbox{valign=m}{\includegraphics[width=1.5cm]{iclr2024/renderings/groundtruth/videoframe_198.png}} 
    \\
    \makecell{\emph{\small{GRF Interlacer}} \\ \emph{\small{prediction}}} & 
    \adjustbox{valign=m}{\includegraphics[width=1.5cm]{iclr2024/renderings/pred/videoframe_0.png}} & 
    \adjustbox{valign=m}{\includegraphics[width=1.5cm]{iclr2024/renderings/pred/videoframe_106.png}} & 
    \adjustbox{valign=m}{\includegraphics[width=1.5cm]{iclr2024/renderings/pred/videoframe_198.png}} 
    \vspace{1mm} \\
    & \small{$t=0$} & \small{$t=1$} & \small{$t=2$}
    \\
    \end{tabular}
\end{minipage}%
\begin{minipage}{0.35\textwidth}
    \centering \vspace{2mm}
    \includegraphics[width=\textwidth]{iclr2024/images/image (3).pdf}
\end{minipage}
\caption{\emph{Left}: NeRF renderings of the predicted dynamics of a bimanual Kuka robot using a dustpan and brush, conditioned on the initial scene and sequence of robot actions.
\emph{Right}: Structural similarity index measure (SSIM) between groundtruth camera frames and predictive NeRF renderings after $100$k training steps, plotted against rollout timestep. Higher is better.
Topological masking with GRFs (\textcolor{red}{ours}) improves the accuracy of dynamics prediction compared to the baselines.} \label{fig:interlacer_plot}
\end{figure}

\section{Limitations and future work}
\begin{enumerate}[leftmargin=*, labelsep=1em]
    \item \textbf{Efficient sparse operations}. We have proved that the time complexity of our algorithm is $\mathcal{O}(N)$ and empirically validated this by counting the number of FLOPs (Fig.~\ref{fig:flops}).
    The algorithm derives its speed from the fact that GRFs are sparse. 
    To fully realise the benefits, one therefore needs an efficient implementation of sparse tensor-tensor multiplication.
    However, at present such operations are not (in general) well-supported above rank 2, limiting batching capabilities for datasets with multiple graph structures and across multiple attention heads. 
    Using asymmetric GRFs partly resolves this by reframing topological masking as a stochastic generalisation of message passing, which obviates sparse linear algebra but at the cost of greater mask estimator variance.
    Moreover, in practice it may not be faster than dense, heavily-optimised matrix-matrix multiplication. 
    We anticipate that the full benefits of topological masking with GRFs will become clearer once the hardware and machine learning libraries for sparse operations catch up with the theory. 
    \item \textbf{Dimensionality reduction of GRFs.} 
    With the above in mind, another interesting avenue for speedups is to reduce the dimensionality of GRFs $\{\widehat{\phi}_\mathcal{G}(v_i)\}_{v_i \in \mathcal{N}} \subset \mathbb{R}^N$, sacrificing their sparsity in favour of shorter lengths.
    This can be achieved without introducing bias into the mask estimate using the celebrated Johnson-Lindenstrauss Transformation \citep[JLT;][]{dasgupta_jlt, dasgupta2003elementary}, which computes random Gaussian projections to get a set of low-dimensional vectors that preserve the original set's dot products with high probability. 
    Given new GRFs $\{\widehat{\phi}_{\mathcal{G}, \textrm{red.}}(v_i)\}_{v_i \in \mathcal{N}} \subset \mathbb{R}^r$, we have that $\widehat{\mathbf{\Phi}}_{\{\mathbf{Q}, \mathbf{K} \}, \mathcal{G}, \textrm{red.}} \subset \mathbb{R}^{N \times rm}$ so that the time complexity of masked attention is $\mathcal{O}(Nmr)$ without relying on sparse operations.
    The drawback is increased mask variance and consequent performance loss; lower-dimensional feature vectors give a less sharp kernel.  
    Another possibility would be a learned (c.f. random) linear projection to reduce GRF dimensionality, eschewing unbiased estimation of $\mathbf{M}_\alpha(\mathcal{G})$ in favour of greater flexibility. 
    We aim to explore these tradeoffs further in future work.
\end{enumerate}
